Splitting method for elliptic equations with line sources

In this paper, we study the mathematical structure and numerical approximation of elliptic problems posed in a (3D) domain $\Omega$ when the right-hand side is a (1D) line source $\Lambda$. The analysis and approximation of such problems is known to be non-standard as the line source causes the solution to be singular. Our main result is a splitting theorem for the solution; we show that the solution admits a split into an explicit, low regularity term capturing the singularity, and a high-regularity correction term $w$ being the solution of a suitable elliptic equation. The splitting theorem states the mathematical structure of the solution; in particular, we find that the solution has anisotropic regularity. More precisely, the solution fails to belong to $H^1$ in the neighbourhood of $\Lambda$, but exhibits piecewise $H^2$-regularity parallel to $\Lambda$. The splitting theorem can further be used to formulate a numerical method in which the solution is approximated via its correction function $w$. This approach has several benefits. Firstly, it recasts the problem as a 3D elliptic problem with a 3D right-hand side belonging to $L^2$, a problem for which the discretizations and solvers are readily available. Secondly, it makes the numerical approximation independent of the discretization of $\Lambda$; thirdly, it improves the approximation properties of the numerical method. We consider here the Galerkin finite element method, and show that the singularity subtraction then recovers optimal convergence rates on uniform meshes, i.e., without needing to refine the mesh around each line segment. The numerical method presented in this paper is therefore well-suited for applications involving a large number of line segments. We illustrate this by treating a dataset (consisting of $\sim 3000$ line segments) describing the vascular system of the brain.

==> Exp1-infinite-line/numerical-test-1.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  $L^2( \Omega)$ &  $H^1( \Omega)$ &  $L^2( \Omega / \Omega_R)$ &  $H^1( \Omega / \Omega_R )$ \\
\midrule
4  &         0.01488 &         0.20694 &                    0.00505 &                     0.09688 \\
8  &         0.00704 &         0.18234 &                    0.00138 &                     0.04461 \\
16 &         0.00344 &         0.17342 &                    0.00041 &                     0.02256 \\
32 &         0.00171 &         0.17032 &                    0.00012 &                     0.01169 \\
64 &         0.00085 &         0.16923 &                    0.00004 &                     0.00575 \\
\toprule
p  &         1.05704 &         0.12749 &                    1.81265 &                     1.05112 \\
\bottomrule
\end{tabular}


==> Exp1-infinite-line/numerical-test-2.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  $L^2( \Omega)$ &  $H^1( \Omega)$ &  $L^2( \Omega / \Omega_R)$ &  $H^1( \Omega / \Omega_R )$ \\
\midrule
4  &         0.00472 &         0.03876 &                    0.00351 &                     0.03786 \\
8  &         0.00130 &         0.01904 &                    0.00087 &                     0.01700 \\
16 &         0.00034 &         0.00943 &                    0.00022 &                     0.00798 \\
32 &         0.00009 &         0.00470 &                    0.00006 &                     0.00392 \\
64 &         0.00002 &         0.00235 &                    0.00001 &                     0.00193 \\
\toprule
p  &         1.90527 &         1.01941 &                    1.98911 &                     1.12306 \\
\bottomrule
\end{tabular}


==> Exp1-infinite-line/sol1-test-horizontal-conv-orig.tex <==
\begin{tabular}{llrrrrrrrr}
\toprule
   &    &  $L^2( \Omega)$ &    nco0 &  $H^1( \Omega)$ &    nco1 &  $L^2( \Omega / \Omega_R)$ &    nco2 &  $H^1( \Omega / \Omega_R)$ &    nco3 \\
N_ver & N_hor &                 &         &                 &         &                            &         &                            &         \\
\midrule
16 & 4  &         1.4e-02 & 0.0e+00 &         1.7e-01 & 0.0e+00 &                    5.4e-03 & 0.0e+00 &                    8.1e-02 & 0.0e+00 \\
   & 8  &         6.0e-03 & 1.2e+00 &         1.6e-01 & 1.7e-01 &                    1.4e-03 & 2.0e+00 &                    4.1e-02 & 9.8e-01 \\
   & 16 &         2.9e-03 & 1.1e+00 &         1.5e-01 & 7.0e-02 &                    3.7e-04 & 1.9e+00 &                    2.1e-02 & 9.4e-01 \\
   & 32 &         1.5e-03 & 9.8e-01 &         1.5e-01 & 2.0e-02 &                    1.6e-04 & 1.2e+00 &                    1.3e-02 & 6.7e-01 \\
   & 64 &         7.8e-04 & 9.0e-01 &         1.5e-01 & 1.0e-02 &                    1.3e-04 & 2.6e-01 &                    1.0e-02 & 3.9e-01 \\
64 & 4  &         1.4e-02 & 0.0e+00 &         1.7e-01 & 0.0e+00 &                    5.5e-03 & 0.0e+00 &                    8.0e-02 & 0.0e+00 \\
   & 8  &         6.0e-03 & 1.2e+00 &         1.5e-01 & 1.7e-01 &                    1.4e-03 & 2.0e+00 &                    4.0e-02 & 1.0e+00 \\
   & 16 &         2.8e-03 & 1.1e+00 &         1.5e-01 & 7.0e-02 &                    3.6e-04 & 1.9e+00 &                    2.0e-02 & 1.0e+00 \\
   & 32 &         1.4e-03 & 1.0e+00 &         1.4e-01 & 2.0e-02 &                    1.1e-04 & 1.8e+00 &                    1.0e-02 & 9.4e-01 \\
   & 64 &         7.0e-04 & 9.9e-01 &         1.4e-01 & 1.0e-02 &                    4.6e-05 & 1.2e+00 &                    5.5e-03 & 9.1e-01 \\
\bottomrule
\end{tabular}


==> Exp1-infinite-line/sol2-test-horizontal-conv-orig.tex <==
\begin{tabular}{llrrrrrrrr}
\toprule
   &    &  $L^2( \Omega)$ &    nco0 &  $H^1( \Omega)$ &    nco1 &  $L^2( \Omega / \Omega_R)$ &    nco2 &  $H^1( \Omega / \Omega_R)$ &    nco3 \\
N_ver & N_hor &                 &         &                 &         &                            &         &                            &         \\
\midrule
16 & 4  &         3.8e-03 & 0.0e+00 &         3.7e-02 & 0.0e+00 &                    3.0e-03 & 0.0e+00 &                    3.1e-02 & 0.0e+00 \\
   & 8  &         9.6e-04 & 2.0e+00 &         1.9e-02 & 1.0e+00 &                    7.2e-04 & 2.0e+00 &                    1.5e-02 & 1.0e+00 \\
   & 16 &         2.4e-04 & 2.0e+00 &         9.4e-03 & 1.0e+00 &                    1.8e-04 & 2.0e+00 &                    7.4e-03 & 1.0e+00 \\
   & 32 &         6.1e-05 & 2.0e+00 &         4.7e-03 & 1.0e+00 &                    4.6e-05 & 2.0e+00 &                    3.8e-03 & 9.8e-01 \\
   & 64 &         1.5e-05 & 2.0e+00 &         2.3e-03 & 1.0e+00 &                    1.1e-05 & 2.0e+00 &                    1.9e-03 & 1.0e+00 \\
64 & 4  &         3.8e-03 & 0.0e+00 &         3.7e-02 & 0.0e+00 &                    3.0e-03 & 0.0e+00 &                    3.1e-02 & 0.0e+00 \\
   & 8  &         9.6e-04 & 2.0e+00 &         1.9e-02 & 1.0e+00 &                    7.2e-04 & 2.0e+00 &                    1.5e-02 & 1.0e+00 \\
   & 16 &         2.4e-04 & 2.0e+00 &         9.4e-03 & 1.0e+00 &                    1.8e-04 & 2.0e+00 &                    7.4e-03 & 1.0e+00 \\
   & 32 &         6.1e-05 & 2.0e+00 &         4.7e-03 & 1.0e+00 &                    4.6e-05 & 2.0e+00 &                    3.8e-03 & 9.8e-01 \\
   & 64 &         1.5e-05 & 2.0e+00 &         2.3e-03 & 1.0e+00 &                    1.1e-05 & 2.0e+00 &                    1.9e-03 & 1.0e+00 \\
\bottomrule
\end{tabular}


==> Exp1-infinite-line/w-test.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  $L^2( \Omega)$ &  $H^1( \Omega)$ &  $L^2( \Omega / \Omega_R)$ &  $H^1( \Omega / \Omega_R)$ \\
h    &                 &                 &                            &                            \\
\midrule
1/4  &         0.00462 &         0.03827 &                    0.00228 &                    0.02767 \\
1/8  &         0.00126 &         0.01893 &                    0.00064 &                    0.01453 \\
1/16 &         0.00033 &         0.00942 &                    0.00016 &                    0.00662 \\
1/32 &         0.00008 &         0.00470 &                    0.00004 &                    0.00325 \\
\midrule
p    &         1.92 &         1.01 &                    1.90 &                    1.03 \\
\bottomrule
\end{tabular}


==> Exp2-finite-line/numerical-test-3.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  $L^2( \Omega)$ &  $H^1( \Omega)$ &  $L^2( \Omega / \Omega_R)$ &  $H^1( \Omega / \Omega_R )$ \\
\midrule
4  &         0.05975 &         1.56898 &                    0.00230 &                     0.02839 \\
8  &         0.02156 &         1.06256 &                    0.00120 &                     0.01747 \\
16 &         0.00782 &         0.83070 &                    0.00010 &                     0.00208 \\
32 &         0.00352 &         0.69483 &                    0.00020 &                     0.00506 \\
p  &         1.47032 &         0.56229 &                    0.94343 &                     0.70090 \\
\bottomrule
\end{tabular}


==> Exp2-finite-line/numerical-test-4.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  $L^2( \Omega)$ &  $H^1( \Omega)$ &  $L^2( \Omega / \Omega_R)$ &  $H^1( \Omega / \Omega_R )$ \\
\midrule
4  &         0.00944 &         0.07905 &                    0.00273 &                     0.03227 \\
8  &         0.00219 &         0.04383 &                    0.00029 &                     0.00471 \\
16 &         0.00060 &         0.01321 &                    0.00015 &                     0.00268 \\
32 &         0.00022 &         0.00816 &                    0.00004 &                     0.00095 \\
p  &         2.10906 &         0.85092 &                    3.23134 &                     2.77727 \\
\bottomrule
\end{tabular}


==> shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

%strongly recommended
\numberwithin{theorem}{section}

% Declare title and authors, without \thanks
\newcommand{\TheTitle}{Elliptic problems with line singularities} 
\newcommand{\TheAuthors}{I. G. Gjerde, K. Kumar, B. Wohlmuth, J. M. Nordbotten}

% Sets running headers as well as PDF title and authors
\headers{\TheTitle}{\TheAuthors}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{{\TheTitle}\thanks{Submitted to the editors DATE.
}}

% Authors: full names plus addresses.
\author{
  Ingeborg Gåseby Gjerde\thanks{Department of Applied Mathematics, University of Bergen
(\email{ingeborg.gjerde@uib.no})}
  \and
  Kundan Kumar\thanks{Department of Applied Mathematics, University of Bergen
(\email{kundan.kumar@uib.no})}
\and
 Barbara Wohlmuth \thanks{Technical University of Munich (\email{ barbara.wohlmuth@ma.tum.de}) }
 \and Jan Martin Nordbotten \thanks{Department of Applied Mathematics, University of Bergen
(\email{jan.nordbotten@uib.no})}
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

